Marking the Wrong Symptoms: Evaluating LLM Watermarks in Medical Texts

Large language models (LLMs) are increasingly integrated into clinical workflows, stressing the need for reliable traceability of model-generated output with watermarking. Yet, most watermarks are evaluated on general-purpose benchmarks, leaving domains like medicine, where small token-level perturbations can result in significant semantic changes, underexplored. In this work, we present the first rigorous study of how LLM watermarks affect medical performance, benchmarking 5 watermarking schemes across 11 LLMs and 7 VLMs on various tasks spanning unimodal and multimodal clinical reasoning. Importantly, we complement existing evaluations by introducing a human-expert-validated pipeline for systematically auditing medical reasoning quality, terminological precision, and induced hallucinations. Our results reveal that watermarking can induce substantial degradation across multiple failure modes, including lexical corruption, hallucinated terminology, and amplified misattribution or omission of image findings. Notably, we find that the absence of domain-specific analyses, combined with aggregate metrics that miss failures inherent to clinical text, can systematically obscure practical watermark-induced degradations. Our findings establish domain-specific evaluation as a prerequisite for the safe deployment of watermarked models in medicine, where current benchmarks can otherwise mask clinically consequential failures.

==> data/acc_at_99tpr.tex <==
% Static design2-style operating-point table.
% Generated once from wm_data.collect_dataset (kept rows only,
% i.e. the same data source as acc_tables_{medqa,medxpertqa_mm}.tex).
% Selection: lowest watermark strength achieving >=99% TPR at 1% FPR.
% Dagger: scheme does not reach 99% TPR; value at max-attainable TPR (>=80%).
% Dash:   scheme cannot reach 80% TPR.
% Red bold: drop > 5 pp.
% Required preamble: \\usepackage{booktabs,xcolor,colortbl}

\newcommand{\drop}[1]{{\color{red!70!black}\textbf{#1}}}
\newcommand{\lowtpr}[1]{#1\textsuperscript{\dag}}

\begin{table}[t]
\centering
\small
\caption{Accuracy change ($\Delta$\,pp) at the deployment-relevant operating point. For each model--scheme pair we report accuracy at the lowest watermark strength achieving $\geq$99\% TPR at 1\% FPR. \textsuperscript{\dag}\,Scheme does not reach 99\% TPR; value shown at maximum attainable TPR ($\geq$80\%). \textbf{---}\,Scheme cannot reach 80\% TPR. \textbf{\color{red!70!black}Bold red}: drop $>$\,5\,pp.}
\label{tab:acc_at_operating_point}
\setlength{\tabcolsep}{5pt}
\begin{tabular}{@{}l c r r r r r@{}}
\toprule
 & Base & \multicolumn{5}{c}{$\Delta$ Accuracy (pp) at $\sim$99\% TPR} \\
\cmidrule(l){3-7}
Model & (\%) & KGW & AAR & PPL & SynthID & DipMark \\
\midrule
\multicolumn{7}{@{}l}{\textit{MedQA (text-only, 4 options)}} \\[2pt]
  \textsc{Llama-3.1-70B} & 91.0 & $-$0.6 & \lowtpr{$-$1.2} & $-$3.1 & \lowtpr{$-$0.7} & \textbf{---} \\
  \textsc{UltraMedical-70B} & 86.6 & $-$1.3 & \lowtpr{$-$1.2} & \drop{$-$16.6} & \drop{$-$23.5} & \textbf{---} \\
  \textsc{Phi-4-14B} & 81.5 & $-$1.2 & \lowtpr{$-$1.8} & $-$4.0 & $-$2.2 & \textbf{---} \\
  \textsc{OpenBioLLM-70B} & 73.8 & \lowtpr{\drop{$-$18.9}} & \textbf{---} & \lowtpr{\drop{$-$6.3}} & \lowtpr{\drop{$-$14.5}} & \textbf{---} \\
  \textsc{Llama-3.1-8B} & 72.8 & \drop{$-$8.2} & \drop{$-$10.8} & $-$4.4 & \drop{$-$24.4} & \lowtpr{\drop{$-$5.5}} \\
  \textsc{Gemma-3-12B} & 68.2 & +0.6 & +1.0 & +0.2 & +0.6 & \lowtpr{+0.3} \\
\midrule
\multicolumn{7}{@{}l}{\textit{MedXpertQA-MM (multimodal, 5 options)}} \\[2pt]
  \textsc{Gemma-4-31B} & 54.9 & $-$0.9 & \lowtpr{$-$1.2} & $-$1.4 & \lowtpr{$-$1.9} & \textbf{---} \\
  \textsc{Qwen-3-VL-32B} & 38.9 & $-$0.4 & $-$0.1 & $-$1.5 & +0.1 & \lowtpr{+0.1} \\
  \textsc{MedGemma-27B} & 32.8 & $-$0.4 & $-$1.0 & $-$0.4 & $-$0.2 & \lowtpr{$-$0.4} \\
  \textsc{Lingshu-32B} & 29.9 & +0.5 & \lowtpr{+0.2} & $-$0.8 & $-$3.4 & \textbf{---} \\
  \textsc{Qwen-3-VL-8B} & 29.8 & $-$0.6 & $-$2.5 & $-$2.9 & $-$3.5 & \lowtpr{$-$0.9} \\
  \textsc{Lingshu-7B} & 24.3 & +0.9 & \lowtpr{$-$0.8} & $-$0.4 & $-$1.3 & \textbf{---} \\
  \textsc{MedGemma-4B} & 24.4 & \lowtpr{$-$2.7} & $-$2.2 & \lowtpr{$-$3.3} & \lowtpr{$-$4.4} & \textbf{---} \\
\bottomrule
\end{tabular}
\end{table}


==> data/all_tables.tex <==
% =============================================================
% Combined accuracy-decomposition tables for 8 models
% Auto-generated from individual tables.tex files
% FPR threshold: 1%
% Required packages: booktabs, graphicx
% =============================================================

% ----- \textsc{Llama-3.1-8B} -----
\begin{table}[htbp]
\centering
\small
\caption{Accuracy decomposition --- \textsc{Llama-3.1-8B} (pass@1, unwatermarked baseline: 72.8\%)}
\label{tab:decomp_Llama3_8B_pass1}
\resizebox{\textwidth}{!}{%
\begin{tabular}{ll rrr}
\toprule
Scheme & Params & Net Acc.\ (\%) & TPR@1\%FPR (\%) & Resp.\ Rate (\%) \\
\midrule
  Unwatermarked & --- & 72.8 & --- & 100.0 \\
\midrule
  AAR & delta=0 & 68.5 & 91.4 & 95.5 \\
  AAR & delta=0.1 & 68.9 & 95.7 & 93.5 \\
  AAR & delta=0.2 & 65.8 & 98.1 & 91.0 \\
  AAR & delta=0.3 & 62.0 & 99.4 & 85.5 \\
  AAR & delta=0.4 & 50.6 & 99.6 & 68.5 \\
  AAR & delta=0.5 & 26.5 & 99.8 & 35.4 \\
\midrule
  DipMark & alpha=0.25 & 68.0 & 69.6 & 94.2 \\
  DipMark & alpha=0.3 & 67.0 & 76.9 & 93.8 \\
  DipMark & alpha=0.35 & 67.8 & 80.9 & 92.8 \\
  DipMark & alpha=0.4 & 68.3 & 83.0 & 93.3 \\
  DipMark & alpha=0.45 & 68.2 & 82.8 & 93.1 \\
  DipMark & alpha=0.5 & 67.2 & 83.8 & 93.3 \\
\midrule
  KGW & delta=0.5 & 70.5 & 18.6 & 96.2 \\
  KGW & delta=1 & 69.6 & 63.0 & 94.8 \\
  KGW & delta=2 & 64.5 & 99.2 & 89.2 \\
  KGW & delta=3 & 57.9 & 100.0 & 81.0 \\
  KGW & delta=4 & 50.8 & 99.9 & 72.7 \\
  KGW & delta=5 & 42.4 & 100.0 & 65.7 \\
\midrule
  PPL & epsilon=0 & 68.3 & 99.1 & 93.6 \\
  PPL & epsilon=0.1 & 66.1 & 99.7 & 90.5 \\
  PPL & epsilon=0.2 & 65.0 & 100.0 & 88.3 \\
  PPL & epsilon=0.3 & 60.2 & 100.0 & 84.7 \\
  PPL & epsilon=0.4 & 56.5 & 100.0 & 79.0 \\
  PPL & epsilon=0.5 & 52.4 & 100.0 & 74.5 \\
\midrule
  SynthID & epsilon=2 & 71.7 & 85.9 & 97.4 \\
  SynthID & epsilon=3 & 65.0 & 98.3 & 90.0 \\
  SynthID & epsilon=4 & 48.4 & 100.0 & 69.4 \\
  SynthID & epsilon=5 & 25.7 & 100.0 & 36.8 \\
  SynthID & epsilon=6 & 4.7 & 100.0 & 7.0 \\
\bottomrule
\end{tabular}
}%
\end{table}

% ----- \textsc{Llama-3.1-70B} -----
\begin{table}[htbp]
\centering
\small
\caption{Accuracy decomposition --- \textsc{Llama-3.1-70B} (pass@1, unwatermarked baseline: 91.0\%)}
\label{tab:decomp_Llama3_70B_pass1}
\resizebox{\textwidth}{!}{%
\begin{tabular}{ll rrr}
\toprule
Scheme & Params & Net Acc.\ (\%) & TPR@1\%FPR (\%) & Resp.\ Rate (\%) \\
\midrule
  Unwatermarked & --- & 91.0 & --- & 100.0 \\
\midrule
  AAR & delta=0 & 89.5 & 37.3 & 100.0 \\
  AAR & delta=0.1 & 90.1 & 47.1 & 100.0 \\
  AAR & delta=0.2 & 89.6 & 55.6 & 100.0 \\
  AAR & delta=0.3 & 90.8 & 64.7 & 100.0 \\
  AAR & delta=0.4 & 89.5 & 73.1 & 100.0 \\
  AAR & delta=0.5 & 89.8 & 80.7 & 100.0 \\
\midrule
  DipMark & alpha=0.25 & 90.2 & 23.2 & 100.0 \\
  DipMark & alpha=0.3 & 90.0 & 27.2 & 100.0 \\
  DipMark & alpha=0.35 & 89.8 & 28.0 & 100.0 \\
  DipMark & alpha=0.4 & 90.2 & 30.4 & 100.0 \\
  DipMark & alpha=0.45 & 89.5 & 29.0 & 100.0 \\
  DipMark & alpha=0.5 & 89.8 & 30.2 & 100.0 \\
\midrule
  KGW & delta=0.5 & 90.1 & 6.4 & 100.0 \\
  KGW & delta=1 & 90.0 & 22.2 & 100.0 \\
  KGW & delta=2 & 89.6 & 70.7 & 100.0 \\
  KGW & delta=3 & 90.0 & 95.2 & 100.0 \\
  KGW & delta=4 & 90.4 & 99.1 & 100.0 \\
  KGW & delta=5 & 89.5 & 99.8 & 100.0 \\
\midrule
  PPL & epsilon=0 & 89.6 & 81.7 & 99.5 \\
  PPL & epsilon=0.1 & 88.2 & 92.8 & 99.1 \\
  PPL & epsilon=0.2 & 89.3 & 97.8 & 99.0 \\
  PPL & epsilon=0.3 & 87.9 & 99.3 & 97.8 \\
  PPL & epsilon=0.4 & 88.1 & 99.7 & 97.4 \\
  PPL & epsilon=0.5 & 85.4 & 99.9 & 95.5 \\
\midrule
  SynthID & epsilon=2 & 89.8 & 38.3 & 100.0 \\
  SynthID & epsilon=3 & 89.6 & 63.9 & 100.0 \\
  SynthID & epsilon=4 & 89.6 & 79.4 & 100.0 \\
  SynthID & epsilon=5 & 90.4 & 87.9 & 100.0 \\
  SynthID & epsilon=6 & 90.3 & 93.4 & 100.0 \\
\bottomrule
\end{tabular}
}%
\end{table}

% ----- \textsc{Gemma-3-12B} -----
\begin{table}[htbp]
\centering
\small
\caption{Accuracy decomposition --- \textsc{Gemma-3-12B} (pass@1, unwatermarked baseline: 66.9\%)}
\label{tab:decomp_Gemma3_12B_pass1}
\resizebox{\textwidth}{!}{%
\begin{tabular}{ll rrr}
\toprule
Scheme & Params & Net Acc.\ (\%) & TPR@1\%FPR (\%) & Resp.\ Rate (\%) \\
\midrule
  Unwatermarked & --- & 66.9 & --- & 99.9 \\
\midrule
  AAR & delta=0 & 69.2 & 96.3 & 100.0 \\
  AAR & delta=0.1 & 68.5 & 98.2 & 100.0 \\
  AAR & delta=0.2 & 69.2 & 99.3 & 100.0 \\
  AAR & delta=0.3 & 68.7 & 99.7 & 100.0 \\
  AAR & delta=0.4 & 69.1 & 99.7 & 99.9 \\
  AAR & delta=0.5 & 68.2 & 100.0 & 100.0 \\
\midrule
  DipMark & alpha=0.25 & 68.3 & 78.3 & 100.0 \\
  DipMark & alpha=0.3 & 69.0 & 84.5 & 100.0 \\
  DipMark & alpha=0.35 & 67.4 & 88.7 & 100.0 \\
  DipMark & alpha=0.4 & 69.8 & 91.3 & 99.9 \\
  DipMark & alpha=0.45 & 67.8 & 90.4 & 100.0 \\
  DipMark & alpha=0.5 & 68.5 & 90.1 & 100.0 \\
\midrule
  KGW & delta=0.5 & 69.2 & 16.9 & 100.0 \\
  KGW & delta=1 & 69.7 & 65.1 & 100.0 \\
  KGW & delta=2 & 68.8 & 99.4 & 100.0 \\
  KGW & delta=3 & 67.8 & 99.9 & 100.0 \\
  KGW & delta=4 & 67.8 & 100.0 & 100.0 \\
  KGW & delta=5 & 68.2 & 100.0 & 100.0 \\
\midrule
  PPL & epsilon=0 & 68.4 & 99.5 & 99.5 \\
  PPL & epsilon=0.1 & 68.8 & 99.9 & 99.6 \\
  PPL & epsilon=0.2 & 67.8 & 100.0 & 98.9 \\
  PPL & epsilon=0.3 & 67.3 & 100.0 & 98.6 \\
  PPL & epsilon=0.4 & 67.3 & 100.0 & 98.3 \\
  PPL & epsilon=0.5 & 66.6 & 100.0 & 97.8 \\
\midrule
  SynthID & epsilon=1 & 69.5 & 1.6 & 100.0 \\
  SynthID & epsilon=2 & 69.5 & 91.1 & 100.0 \\
  SynthID & epsilon=3 & 69.5 & 98.9 & 100.0 \\
  SynthID & epsilon=4 & 68.8 & 100.0 & 99.9 \\
  SynthID & epsilon=5 & 67.9 & 100.0 & 99.9 \\
  SynthID & epsilon=6 & 67.8 & 100.0 & 99.8 \\
\bottomrule
\end{tabular}
}%
\end{table}

% ----- \textsc{Phi-4-14B} -----
\begin{table}[htbp]
\centering
\small
\caption{Accuracy decomposition --- \textsc{Phi-4-14B} (pass@1, unwatermarked baseline: 81.5\%)}
\label{tab:decomp_Phi4_pass1}
\resizebox{\textwidth}{!}{%
\begin{tabular}{ll rrr}
\toprule
Scheme & Params & Net Acc.\ (\%) & TPR@1\%FPR (\%) & Resp.\ Rate (\%) \\
\midrule
  Unwatermarked & --- & 81.5 & --- & 99.7 \\
\midrule
  AAR & delta=0 & 82.5 & 70.0 & 99.2 \\
  AAR & delta=0.1 & 80.9 & 80.0 & 99.1 \\
  AAR & delta=0.2 & 81.3 & 86.0 & 99.1 \\
  AAR & delta=0.3 & 81.6 & 92.0 & 99.4 \\
  AAR & delta=0.4 & 80.8 & 96.2 & 99.2 \\
  AAR & delta=0.5 & 79.7 & 98.1 & 99.2 \\
\midrule
  DipMark & alpha=0.25 & 81.1 & 46.6 & 99.3 \\
  DipMark & alpha=0.3 & 80.5 & 51.3 & 99.0 \\
  DipMark & alpha=0.35 & 81.8 & 55.5 & 99.6 \\
  DipMark & alpha=0.4 & 81.2 & 57.6 & 99.3 \\
  DipMark & alpha=0.45 & 80.8 & 59.2 & 99.2 \\
  DipMark & alpha=0.5 & 81.1 & 59.8 & 99.6 \\
\midrule
  KGW & delta=0.5 & 81.8 & 5.9 & 99.6 \\
  KGW & delta=1 & 82.2 & 27.5 & 99.8 \\
  KGW & delta=2 & 80.7 & 87.3 & 99.5 \\
  KGW & delta=3 & 80.3 & 99.2 & 99.7 \\
  KGW & delta=4 & 80.7 & 99.9 & 99.6 \\
  KGW & delta=5 & 79.8 & 99.9 & 99.6 \\
\midrule
  PPL & epsilon=0 & 78.8 & 90.8 & 96.7 \\
  PPL & epsilon=0.1 & 78.8 & 96.7 & 96.7 \\
  PPL & epsilon=0.2 & 79.1 & 99.7 & 96.4 \\
  PPL & epsilon=0.3 & 77.5 & 99.8 & 95.0 \\
  PPL & epsilon=0.4 & 75.0 & 99.9 & 94.0 \\
  PPL & epsilon=0.5 & 74.2 & 100.0 & 92.8 \\
\midrule
  SynthID & epsilon=1 & 81.8 & 0.9 & 99.6 \\
  SynthID & epsilon=2 & 81.2 & 48.4 & 99.2 \\
  SynthID & epsilon=3 & 80.8 & 84.5 & 99.4 \\
  SynthID & epsilon=4 & 80.0 & 97.2 & 99.5 \\
  SynthID & epsilon=5 & 79.3 & 99.1 & 99.5 \\
  SynthID & epsilon=6 & 77.0 & 99.7 & 98.9 \\
\bottomrule
\end{tabular}
}%
\end{table}

% ----- \textsc{Mixtral} -----
\begin{table}[htbp]
\centering
\small
\caption{Accuracy decomposition --- \textsc{Mixtral} (pass@1, unwatermarked baseline: 60.1\%)}
\label{tab:decomp_Mixtral_pass1}
\resizebox{\textwidth}{!}{%
\begin{tabular}{ll rrr}
\toprule
Scheme & Params & Net Acc.\ (\%) & TPR@1\%FPR (\%) & Resp.\ Rate (\%) \\
\midrule
  Unwatermarked & --- & 60.1 & --- & 96.5 \\
\midrule
  AAR & delta=0 & 61.2 & 53.6 & 96.9 \\
  AAR & delta=0.1 & 61.1 & 63.3 & 95.9 \\
  AAR & delta=0.2 & 60.5 & 71.2 & 95.9 \\
  AAR & delta=0.3 & 60.8 & 77.6 & 95.9 \\
  AAR & delta=0.4 & 58.9 & 82.3 & 95.8 \\
  AAR & delta=0.5 & 60.8 & 87.5 & 95.5 \\
\midrule
  DipMark & alpha=0.25 & 60.6 & 30.4 & 95.7 \\
  DipMark & alpha=0.3 & 60.5 & 34.4 & 96.6 \\
  DipMark & alpha=0.35 & 61.4 & 38.8 & 96.2 \\
  DipMark & alpha=0.4 & 60.2 & 39.1 & 95.6 \\
  DipMark & alpha=0.45 & 59.3 & 41.2 & 95.7 \\
  DipMark & alpha=0.5 & 60.5 & 41.1 & 96.0 \\
\midrule
  KGW & delta=0.5 & 59.5 & 4.5 & 95.3 \\
  KGW & delta=1 & 59.9 & 18.2 & 96.1 \\
  KGW & delta=2 & 58.1 & 66.1 & 94.6 \\
  KGW & delta=3 & 60.5 & 90.5 & 95.0 \\
  KGW & delta=4 & 58.1 & 97.8 & 92.3 \\
  KGW & delta=5 & 56.4 & 99.4 & 89.5 \\
\midrule
  PPL & epsilon=0 & 59.5 & 68.5 & 95.3 \\
  PPL & epsilon=0.1 & 58.1 & 81.7 & 94.5 \\
  PPL & epsilon=0.2 & 58.5 & 90.4 & 93.5 \\
  PPL & epsilon=0.3 & 56.6 & 95.9 & 91.0 \\
  PPL & epsilon=0.4 & 56.2 & 98.0 & 89.1 \\
  PPL & epsilon=0.5 & 53.0 & 99.2 & 85.4 \\
\midrule
  SynthID & epsilon=1 & 61.5 & 0.3 & 96.7 \\
  SynthID & epsilon=2 & 61.1 & 33.5 & 96.1 \\
  SynthID & epsilon=3 & 59.3 & 59.8 & 94.3 \\
  SynthID & epsilon=4 & 58.1 & 77.0 & 92.5 \\
  SynthID & epsilon=5 & 57.8 & 88.2 & 92.0 \\
  SynthID & epsilon=6 & 56.0 & 94.2 & 88.6 \\
\bottomrule
\end{tabular}
}%
\end{table}

% ----- \textsc{Minitron-8B} -----
\begin{table}[htbp]
\centering
\small
\caption{Accuracy decomposition --- \textsc{Minitron-8B} (pass@1, unwatermarked baseline: 56.0\%)}
\label{tab:decomp_Minitron_8B_pass1}
\resizebox{\textwidth}{!}{%
\begin{tabular}{ll rrr}
\toprule
Scheme & Params & Net Acc.\ (\%) & TPR@1\%FPR (\%) & Resp.\ Rate (\%) \\
\midrule
  Unwatermarked & --- & 56.0 & --- & 99.7 \\
\midrule
  AAR & delta=0 & 56.0 & 87.4 & 99.8 \\
  AAR & delta=0.1 & 55.9 & 92.0 & 99.7 \\
  AAR & delta=0.2 & 54.9 & 95.7 & 99.6 \\
  AAR & delta=0.3 & 56.1 & 98.5 & 99.5 \\
  AAR & delta=0.4 & 55.8 & 99.0 & 99.5 \\
  AAR & delta=0.5 & 55.3 & 99.3 & 98.8 \\
\midrule
  DipMark & alpha=0.25 & 56.1 & 61.5 & 99.8 \\
  DipMark & alpha=0.3 & 56.4 & 66.2 & 99.9 \\
  DipMark & alpha=0.35 & 55.7 & 72.2 & 99.8 \\
  DipMark & alpha=0.4 & 55.9 & 74.5 & 99.8 \\
  DipMark & alpha=0.45 & 55.8 & 76.3 & 99.9 \\
  DipMark & alpha=0.5 & 55.7 & 75.4 & 99.9 \\
\midrule
  KGW & delta=0.5 & 56.2 & 9.7 & 100.0 \\
  KGW & delta=1 & 55.9 & 43.6 & 99.9 \\
  KGW & delta=2 & 55.6 & 93.8 & 99.9 \\
  KGW & delta=3 & 54.8 & 99.8 & 99.9 \\
  KGW & delta=4 & 54.5 & 99.9 & 99.7 \\
  KGW & delta=5 & 54.5 & 100.0 & 99.8 \\
\midrule
  PPL & epsilon=0 & 55.8 & 95.7 & 99.7 \\
  PPL & epsilon=0.1 & 55.5 & 98.9 & 99.5 \\
  PPL & epsilon=0.2 & 55.4 & 99.5 & 99.4 \\
  PPL & epsilon=0.3 & 55.1 & 99.9 & 99.1 \\
  PPL & epsilon=0.4 & 54.5 & 99.9 & 98.2 \\
  PPL & epsilon=0.5 & 53.9 & 100.0 & 97.2 \\
\midrule
  SynthID & epsilon=1 & 56.3 & 1.0 & 99.7 \\
  SynthID & epsilon=2 & 56.2 & 74.1 & 99.9 \\
  SynthID & epsilon=3 & 55.8 & 97.0 & 99.8 \\
  SynthID & epsilon=4 & 55.2 & 99.4 & 99.4 \\
  SynthID & epsilon=5 & 54.3 & 99.9 & 96.9 \\
  SynthID & epsilon=6 & 48.4 & 100.0 & 86.8 \\
\bottomrule
\end{tabular}
}%
\end{table}

% ----- \textsc{OpenBioLLM-70B} -----
\begin{table}[htbp]
\centering
\small
\caption{Accuracy decomposition --- \textsc{OpenBioLLM-70B} (pass@1, unwatermarked baseline: 73.8\%)}
\label{tab:decomp_OpenBioLLM_70B_pass1}
\resizebox{\textwidth}{!}{%
\begin{tabular}{ll rrr}
\toprule
Scheme & Params & Net Acc.\ (\%) & TPR@1\%FPR (\%) & Resp.\ Rate (\%) \\
\midrule
  Unwatermarked & --- & 73.8 & --- & 94.6 \\
\midrule
  AAR & delta=0 & 76.0 & 36.6 & 95.5 \\
  AAR & delta=0.1 & 74.5 & 45.3 & 95.3 \\
  AAR & delta=0.2 & 73.7 & 51.7 & 94.8 \\
  AAR & delta=0.3 & 74.9 & 59.1 & 96.0 \\
  AAR & delta=0.4 & 72.7 & 66.7 & 93.6 \\
  AAR & delta=0.5 & 72.0 & 76.1 & 93.3 \\
\midrule
  DipMark & alpha=0.25 & 74.5 & 17.4 & 93.5 \\
  DipMark & alpha=0.3 & 73.7 & 20.2 & 93.2 \\
  DipMark & alpha=0.35 & 73.4 & 21.7 & 93.8 \\
  DipMark & alpha=0.4 & 71.7 & 24.1 & 92.0 \\
  DipMark & alpha=0.45 & 72.2 & 25.6 & 92.5 \\
  DipMark & alpha=0.5 & 72.0 & 25.4 & 91.9 \\
\midrule
  KGW & delta=0.5 & 74.5 & 3.1 & 94.8 \\
  KGW & delta=1 & 74.9 & 11.4 & 95.0 \\
  KGW & delta=2 & 73.4 & 51.4 & 93.3 \\
  KGW & delta=3 & 69.0 & 85.5 & 90.2 \\
  KGW & delta=4 & 63.1 & 95.9 & 84.8 \\
  KGW & delta=5 & 54.9 & 98.8 & 76.2 \\
\midrule
  PPL & epsilon=0 & 73.4 & 57.2 & 94.2 \\
  PPL & epsilon=0.1 & 73.5 & 73.9 & 93.5 \\
  PPL & epsilon=0.2 & 71.9 & 86.6 & 91.2 \\
  PPL & epsilon=0.3 & 69.8 & 92.7 & 88.8 \\
  PPL & epsilon=0.4 & 69.2 & 95.4 & 88.5 \\
  PPL & epsilon=0.5 & 67.5 & 97.5 & 87.2 \\
\midrule
  SynthID & epsilon=1 & 77.7 & 0.8 & 96.7 \\
  SynthID & epsilon=2 & 75.9 & 22.9 & 96.2 \\
  SynthID & epsilon=3 & 73.9 & 48.1 & 94.2 \\
  SynthID & epsilon=4 & 71.2 & 70.5 & 91.2 \\
  SynthID & epsilon=5 & 67.2 & 83.5 & 87.4 \\
  SynthID & epsilon=6 & 59.2 & 93.3 & 81.0 \\
\bottomrule
\end{tabular}
}%
\end{table}

% ----- \textsc{UltraMedical-70B} -----
\begin{table}[htbp]
\centering
\small
\caption{Accuracy decomposition --- \textsc{UltraMedical-70B} (pass@1, unwatermarked baseline: 66.2\%)}
\label{tab:decomp_UltraMedical_70B_pass1}
\resizebox{\textwidth}{!}{%
\begin{tabular}{ll rrr}
\toprule
Scheme & Params & Net Acc.\ (\%) & TPR@1\%FPR (\%) & Resp.\ Rate (\%) \\
\midrule
  Unwatermarked & --- & 66.2 & --- & 76.5 \\
\midrule
  AAR & delta=0 & 75.9 & 67.8 & 87.1 \\
  AAR & delta=0.1 & 76.6 & 76.5 & 87.9 \\
  AAR & delta=0.2 & 77.3 & 84.4 & 88.9 \\
  AAR & delta=0.3 & 76.3 & 90.5 & 88.8 \\
  AAR & delta=0.4 & 76.5 & 93.5 & 88.2 \\
  AAR & delta=0.5 & 75.8 & 95.6 & 88.5 \\
\midrule
  DipMark & alpha=0.25 & 65.4 & 42.3 & 75.0 \\
  DipMark & alpha=0.3 & 66.8 & 48.5 & 76.8 \\
  DipMark & alpha=0.35 & 66.0 & 53.0 & 75.4 \\
  DipMark & alpha=0.4 & 66.9 & 57.0 & 76.8 \\
  DipMark & alpha=0.45 & 67.0 & 56.5 & 78.0 \\
  DipMark & alpha=0.5 & 67.0 & 57.7 & 76.2 \\
\midrule
  KGW & delta=0.5 & 63.6 & 11.7 & 72.0 \\
  KGW & delta=1 & 59.1 & 41.2 & 68.1 \\
  KGW & delta=2 & 58.0 & 91.4 & 67.5 \\
  KGW & delta=3 & 61.1 & 99.1 & 71.2 \\
  KGW & delta=4 & 65.8 & 100.0 & 77.3 \\
  KGW & delta=5 & 62.5 & 100.0 & 74.0 \\
\midrule
  PPL & epsilon=0 & 60.5 & 94.4 & 69.7 \\
  PPL & epsilon=0.1 & 59.2 & 97.7 & 67.1 \\
  PPL & epsilon=0.2 & 52.7 & 99.3 & 61.5 \\
  PPL & epsilon=0.3 & 48.6 & 98.7 & 56.9 \\
  PPL & epsilon=0.4 & 42.6 & 99.1 & 50.5 \\
  PPL & epsilon=0.5 & 37.5 & 99.2 & 43.9 \\
\midrule
  SynthID & epsilon=1 & 68.0 & 1.4 & 77.5 \\
  SynthID & epsilon=2 & 64.2 & 67.4 & 73.1 \\
  SynthID & epsilon=3 & 63.4 & 89.2 & 73.0 \\
  SynthID & epsilon=4 & 64.3 & 96.3 & 74.3 \\
  SynthID & epsilon=5 & 63.3 & 98.8 & 73.5 \\
  SynthID & epsilon=6 & 53.5 & 99.2 & 62.2 \\
\bottomrule
\end{tabular}
}%
\end{table}


==> data/full_taskA_MedQA.tex <==
\begin{sidewaystable}
\centering
\scriptsize
\setlength{\tabcolsep}{1.5pt}
\begin{threeparttable}
\caption{\textbf{Full reasoning audit on MedQA, all $7$ LLMs, at $\geq 99\%$ TPR.} Scheme rows are paired-bootstrap $\Delta$ vs.\ the unwatermarked baseline over $N{=}2000$ paired completions; VigFab and FabRatio are WM/Base ratios and Major\% is absolute. $^{*}\,p{<}0.01$ (sign-flip permutation, $n{=}5000$); ``--'': base rate too low for a stable ratio.}\label{tab:taskA_full_MedQA}
\begin{tabular}{llrrrrrrrrrrrrr}
\toprule
Model & Scheme & $\Delta$Acc & $\Delta$ConfErr & $\Delta$F\&C & $\Delta$Spell/100 & $\Delta$Fab/100 & $\Delta$Contr & $\Delta$VigFab & $\Delta$Misread & $\Delta$Fmt & $\Delta$Ling & $\Delta$Misapp/100 & Major\% & FabRatio \\
\midrule
\textsc{Llama-3.1-8B} & Unwatermarked & 73.3 & 35.3 & 29.6 & 0.8 & 1.4 & 22.6 & 5.8 & 6.6 & 0.9 & 0.1 & 23.2 & -- & 1.0$\times$ \\
 & AAR & -0.6 & +8.1* & +7.4* & +5.8* & +4.1* & +6.1* & +5.5* & +3.2* & +1.5* & +6.1* & +1.5 & 31.9 & 2.1$\times$* \\
 & DipMark & -1.6 & -0.7 & +1.0 & +0.9 & +1.0 & +3.1 & +1.3 & +3.4* & -0.3 & +0.5 & -2.0 & 29.2 & 1.6$\times$ \\
 & KGW & -2.3 & +3.0 & +2.4 & +1.8* & +2.2* & +5.1* & +1.7 & +1.6 & +0.5 & +0.3 & +0.4 & 29.0 & 1.0$\times$ \\
 & PPL & -0.7 & +5.4 & +4.3 & +24.6* & +1.0 & +4.2 & +0.5 & +3.8* & +0.3 & +3.4* & -0.7 & 29.8 & 1.6$\times$ \\
 & SynthID & -2.0 & +3.0 & +2.2 & +2.1* & +1.5 & +4.0 & +3.7* & +2.6 & +1.5 & +0.7 & +1.0 & 33.5 & 1.2$\times$ \\
\textsc{Llama-3.1-70B} & Unwatermarked & 91.8 & 6.9 & 8.1 & 0.4 & 0.1 & 5.8 & 0.4 & 1.0 & 0.0 & 0.0 & 2.4 & -- & 1.0$\times$ \\
 & AAR & -1.2 & -0.5 & +0.1 & +0.3 & 0.0 & +0.1 & +0.1 & +0.5 & 0.0 & +0.1 & -0.5 & 4.1 & -- \\
 & DipMark & -1.2 & +1.4 & +1.5 & -0.1 & -0.1 & +1.4 & -0.2 & +0.2 & +0.2 & 0.0 & +0.1 & 4.0 & -- \\
 & KGW & -1.3 & +1.8 & +1.9 & +1.0 & 0.0 & +1.6 & +0.4 & +0.3 & +0.1 & +0.1 & +0.9 & 5.1 & 1.0$\times$ \\
 & PPL & -1.8 & +3.3* & +7.5* & +89.4* & +1.9* & +2.1 & +0.3 & +3.5* & +0.6 & +30.9* & +0.3 & 5.0 & -- \\
 & SynthID & -0.9 & +2.0 & +1.2 & +6.5* & +0.2 & +0.9 & +0.4 & -0.1 & +0.1 & +3.4* & 0.0 & 5.9 & 0.0$\times$ \\
\textsc{Gemma-3-12B} & Unwatermarked & 67.0 & 29.2 & 22.5 & 0.7 & 1.3 & 20.4 & 3.4 & 4.5 & 0.0 & 0.0 & 19.8 & -- & 1.0$\times$ \\
 & AAR & +1.3 & +2.5 & +3.4 & +0.2 & +0.4 & +3.2 & -0.7 & +0.3 & +0.2 & 0.0 & +1.4 & 21.0 & 0.9$\times$ \\
 & DipMark & +1.8 & -1.0 & +1.1 & -0.3 & +0.2 & +1.7 & -0.4 & -0.7 & +0.4 & +0.1 & +1.5 & 20.9 & 0.4$\times$ \\
 & KGW & +1.5 & +0.7 & +1.7 & +0.1 & 0.0 & +1.9 & +1.0 & +0.1 & +0.1 & 0.0 & -0.7 & 22.4 & 1.3$\times$ \\
 & PPL & +1.5 & +2.5 & +3.2 & +20.8* & +1.2 & +2.1 & +0.1 & +3.9* & +0.6 & +3.7* & +0.7 & 23.1 & 1.1$\times$ \\
 & SynthID & +1.9 & +3.0 & +4.5* & +2.6* & +0.3 & +3.0 & +1.1 & +0.5 & +0.2 & +0.1 & -0.9 & 22.9 & 1.1$\times$ \\
\textsc{OpenBioLLM-70B} & Unwatermarked & 73.6 & 13.9 & 12.9 & 0.6 & 0.0 & 8.6 & 2.2 & 2.2 & 14.8 & 0.1 & 10.9 & -- & 1.0$\times$ \\
 & AAR & -0.2 & +6.6* & +4.4* & +0.9 & +0.9* & +3.8* & +1.7 & +0.6 & +4.0 & +0.9 & +0.5 & 20.6 & 0.9$\times$ \\
 & DipMark & -1.1 & +2.3 & +1.5 & +0.3 & +0.4 & +1.4 & +0.8 & +1.2 & +5.3* & +0.1 & -0.4 & 18.6 & 1.1$\times$ \\
 & KGW & -17.4* & +11.4* & +4.2* & +5.2* & +1.9* & +9.3* & +7.0* & +6.6* & +20.2* & +0.3 & +3.8 & 24.6 & 3.5$\times$* \\
 & PPL & -7.7* & +7.1* & +6.7* & +51.5* & +2.1* & +4.1* & +3.9* & +4.6* & +13.0* & +8.5* & -0.1 & 23.0 & 1.9$\times$ \\
 & SynthID & -11.4* & +24.0* & +14.6* & +25.9* & +13.6* & +12.3* & +13.0* & +7.9* & +15.5* & +13.8* & +5.3* & 27.8 & 6.6$\times$* \\
Ultramedical 70B & Unwatermarked & 86.6 & 11.0 & 11.8 & 1.0 & 0.0 & 8.0 & 0.5 & 1.5 & 23.2 & 2.2 & 4.4 & -- & 1.0$\times$ \\
 & AAR & -1.5 & +2.3 & +2.5 & +0.5 & +0.4 & +4.5* & +0.9 & +1.8* & -13.1* & -0.9 & 0.0 & 10.7 & 1.0$\times$ \\
 & DipMark & +1.2 & +2.0 & +1.7 & 0.0 & 0.0 & +0.9 & +0.9 & +0.2 & -1.7 & +0.7 & -0.6 & 10.2 & 0.5$\times$ \\
 & KGW & -1.5 & +2.0 & +1.8 & +0.4 & +0.2 & +0.9 & +1.0 & +0.4 & +10.3* & +1.4 & -0.3 & 10.3 & 3.0$\times$ \\
 & PPL & -39.5* & +6.5* & +0.2 & +97.8* & +1.3* & +2.7 & +2.4* & +7.4* & +27.6* & +22.3* & +0.5 & 11.4 & 22.0$\times$* \\
 & SynthID & -9.2* & +3.9 & +3.3 & +6.1* & +0.5 & +3.5* & +1.3* & +2.7* & +4.1 & +4.1* & +1.0 & 10.1 & 1.2$\times$ \\
\textsc{Phi-4-14B} & Unwatermarked & 81.4 & 12.3 & 11.4 & 0.1 & 0.3 & 7.8 & 1.6 & 2.0 & 0.4 & 0.0 & 9.8 & -- & 1.0$\times$ \\
 & AAR & -2.5 & +6.2* & +6.5* & +1.5* & +1.8* & +4.4* & +2.9* & +2.2* & +0.6 & +0.2 & +3.8* & 11.3 & 14.0$\times$* \\
 & DipMark & -0.9 & +3.9* & +3.6* & +0.3 & +0.1 & +2.0 & +0.6 & -0.1 & +0.2 & 0.0 & +2.0 & 10.8 & 0.8$\times$ \\
 & KGW & -0.7 & +9.2* & +9.5* & +2.2* & +1.5* & +5.5* & +3.4* & +3.6* & +0.2 & +0.1 & +3.2 & 14.2 & 3.0$\times$* \\
 & PPL & -8.6* & +10.0* & +9.6* & +69.6* & +3.8* & +5.2* & +3.2* & +4.0* & +5.4* & +10.4* & +3.8 & 13.4 & 18.0$\times$* \\
 & SynthID & -3.2* & +13.7* & +14.9* & +10.6* & +6.6* & +9.4* & +6.8* & +5.5* & +0.7 & +3.9* & +7.2* & 15.4 & 7.6$\times$* \\
\textsc{BioMistral-7B} & Unwatermarked & 40.8 & 1.1 & 1.3 & 0.3 & 0.4 & 1.8 & 1.9 & 0.7 & 7.4 & 0.0 & 2.6 & -- & 1.0$\times$ \\
 & AAR & -1.1 & +21.2* & +8.4* & +5.2* & +12.3* & +8.6* & +13.3* & +8.2* & +7.3* & +3.4* & +8.8* & 25.1 & 14.0$\times$* \\
 & DipMark & -1.3 & +7.9* & +3.4* & +0.9 & +1.4 & +5.8* & +3.8* & +2.6* & -6.5* & +0.2 & +2.0 & 11.5 & 4.9$\times$* \\
 & KGW & -38.7* & +27.8 & -0.6 & +19.6* & +9.1* & +16.9* & +13.8* & +11.7* & +28.3* & +3.9* & +10.4* & 48.9 & 18.1$\times$* \\
 & PPL & -5.0* & +13.2* & +5.0* & +18.5* & +1.9* & +8.6* & +5.2* & +5.3* & +11.1* & +2.0* & +3.4* & 11.8 & 9.5$\times$* \\
 & SynthID & -30.4* & +10.5* & +3.4* & +82.3* & +153.4* & +1.8 & +30.4* & +8.2* & +66.7* & +69.0* & +3.3* & 63.0 & 93.0$\times$* \\
\bottomrule
\end{tabular}
\begin{tablenotes}
\footnotesize
\item Single-response axes (per $100$ questions where suffixed): ConfErr (confident error, on BOTH-CORRECT pairs), F\&C (faulty-but-correct: correct letter $+\geq 1$ defect), Spell/100, Fab/100 (fabricated entities), Contr (within-response contradiction), VigFab (vignette fabrication), Misread (clue misread), Fmt (format/termination failure), Ling (linguistic corruption), Misapp/100 (misapplied real terms). Pairwise: Major\% (MAJOR divergence on BOTH-CORRECT pairs), FabRatio (WM/Base vignette-fabrication rate).
\end{tablenotes}
\end{threeparttable}
\end{sidewaystable}

==> data/full_taskA_MedXpertQA_MM.tex <==
\begin{sidewaystable}
\centering
\scriptsize
\setlength{\tabcolsep}{1.5pt}
\begin{threeparttable}
\caption{\textbf{Full reasoning audit on MedXpertQA-MM, all $7$ VLMs, at $\geq 99\%$ TPR.} Includes the multimodal image-grounding columns (Net\%, Sup, Con). Scheme rows are paired-bootstrap $\Delta$ vs.\ the unwatermarked baseline over $N{=}2000$ paired completions; VigFab and FabRatio are WM/Base ratios and Major\% is absolute. $^{*}\,p{<}0.01$ (sign-flip permutation, $n{=}5000$); ``--'': base rate too low for a stable ratio.}\label{tab:taskA_full_MedXpertQA_MM}
\begin{tabular}{llrrrrrrrrrrrrrrrr}
\toprule
Model & Scheme & $\Delta$Acc & $\Delta$ConfErr & $\Delta$F\&C & $\Delta$Spell/100 & $\Delta$Fab/100 & $\Delta$Net\% & $\Delta$Contr & $\Delta$VigFab & $\Delta$Misread & $\Delta$Fmt & $\Delta$Ling & $\Delta$Misapp/100 & $\Delta$Sup & $\Delta$Con & Major\% & FabRatio \\
\midrule
\textsc{Gemma-4-31B} & Unwatermarked & 56.2 & 12.2 & 9.2 & 0.1 & 0.3 & 2 & 5.0 & 0.8 & 1.9 & 0.1 & 0.0 & 3.0 & 2.55 & 0.53 & -- & 1.0$\times$ \\
 & AAR & -0.6 & -0.6 & -0.3 & +0.9 & +0.3 & +1 & +0.7 & +0.1 & -0.1 & +0.1 & +0.8 & -0.3 & -0.01 & -0.03 & 6.0 & 3.0$\times$ \\
 & DipMark & -0.1 & -1.0 & -0.3 & +0.5 & +0.2 & +2 & +0.5 & -0.5 & 0.0 & +0.1 & 0.0 & +1.4 & +0.02 & -0.03 & 3.6 & 2.0$\times$ \\
 & KGW & +0.2 & -1.7 & -0.3 & +1.8* & +0.2 & +1 & +1.7 & -0.2 & +0.3 & +0.2 & +1.5* & +0.7 & +0.04 & +0.01 & 6.8 & 0.5$\times$ \\
 & PPL & -0.9 & +1.6 & +3.1 & +34.5* & +1.5* & -2 & +1.8 & -0.3 & +3.4* & +2.1* & +22.5* & -0.5 & -0.04 & -0.01 & 5.0 & 6.0$\times$* \\
 & SynthID & -1.0 & +0.4 & -0.3 & +7.6* & +0.8 & +3 & +1.0 & -0.1 & -0.3 & +0.1 & +11.0* & -0.1 & +0.02 & -0.04 & 6.8 & 4.0$\times$ \\
\textsc{Lingshu-7B} & Unwatermarked & 23.9 & 55.3 & 13.7 & 0.4 & 1.5 & 0 & 17.0 & 3.5 & 7.6 & 0.8 & 0.5 & 17.6 & 1.15 & 0.77 & -- & 1.0$\times$ \\
 & AAR & -0.5 & +13.8 & +3.7 & +5.4* & +12.9* & -67* & +3.5 & +7.9* & +3.8* & +2.0* & +3.5* & +3.5 & -0.15* & +0.09 & 33.0 & 2.8$\times$* \\
 & DipMark & +1.0 & +5.4 & +1.4 & +0.1 & +0.3 & -6 & +2.7 & +0.1 & 0.0 & -0.1 & +0.1 & +0.5 & -0.02 & -0.00 & 22.6 & 1.0$\times$ \\
 & KGW & -0.8 & +28.6* & +6.0 & +16.2* & +13.2* & -103* & +20.2* & +10.4* & +11.0* & +5.4* & +4.6* & +12.2* & -0.12 & +0.37* & 42.9 & 3.6$\times$* \\
 & PPL & -0.6 & +7.3 & +2.3 & +37.9* & +3.9* & -44 & +3.9 & +3.0* & +7.9* & +5.1* & +8.4* & -1.3 & -0.13* & +0.03 & 20.0 & 2.4$\times$* \\
 & SynthID & -2.1 & +26.2* & +5.5* & +18.9* & +39.2* & -105* & +13.2* & +16.8* & +8.5* & +7.7* & +13.5* & +12.0* & -0.14* & +0.28* & 30.5 & 7.0$\times$* \\
\textsc{Lingshu-32B} & Unwatermarked & 31.1 & 40.8 & 15.1 & 0.8 & 0.1 & 1 & 9.6 & 2.0 & 3.7 & 0.4 & 0.1 & 8.2 & 1.38 & 0.68 & -- & 1.0$\times$ \\
 & AAR & -1.8 & +9.2 & +1.3 & +2.9* & +5.4* & -46* & +4.8* & +5.5* & +3.4* & +2.5* & +3.5* & +3.0 & -0.15* & +0.17* & 18.0 & 3.8$\times$* \\
 & DipMark & +0.4 & -1.2 & -1.0 & -0.1 & +0.4 & -16 & +1.0 & +0.1 & +0.6 & -0.2 & 0.0 & +0.4 & -0.05 & +0.07 & 15.3 & 0.8$\times$ \\
 & KGW & -4.0 & +10.1 & -0.1 & +1.9* & +1.8* & -39* & +8.9* & +2.4* & +4.8* & +1.1 & +0.8 & +4.7* & -0.05 & +0.23* & 14.4 & 1.8$\times$ \\
 & PPL & -2.4 & -3.2 & -2.0 & +27.4* & +0.8 & -26 & +2.3 & +1.2 & +7.1* & +6.7* & +5.3* & +0.8 & -0.06 & +0.12* & 11.2 & 2.2$\times$* \\
 & SynthID & -3.8 & +6.7 & +2.0 & +23.9* & +13.7* & -56* & +16.2* & +9.8* & +9.5* & +8.8* & +13.2* & +8.4* & -0.12 & +0.28* & 21.7 & 4.9$\times$* \\
\textsc{MedGemma-4B} & Unwatermarked & 24.1 & 56.9 & 16.5 & 1.0 & 1.9 & 0 & 29.7 & 3.5 & 9.0 & 7.7 & 0.0 & 16.5 & 1.24 & 1.11 & -- & 1.0$\times$ \\
 & AAR & -1.0 & +13.0* & +1.2 & +3.4* & +6.5* & -108 & +2.1 & +7.4* & +3.3 & +11.2* & +4.6* & +8.7* & +0.15* & +0.29* & 38.3 & 3.1$\times$* \\
 & DipMark & +0.2 & +11.6 & +1.6 & +0.2 & +0.7 & -103 & -0.9 & +0.1 & -0.2 & -0.2 & +0.3 & +1.4 & -0.08 & +0.06 & 35.0 & 1.2$\times$ \\
 & KGW & -2.6 & +19.2* & +0.6 & +15.4* & +8.9* & -266* & +11.2* & +6.5* & +7.4* & +13.1* & +3.5* & +11.8* & -0.01 & +0.32* & 31.7 & 3.1$\times$* \\
 & PPL & -1.7 & +8.3 & 0.0 & +43.6* & +6.0* & -46 & +4.2 & +3.1* & +8.2* & +8.0* & +9.7* & +4.5 & -0.01 & +0.05 & 34.7 & 2.1$\times$* \\
 & SynthID & -3.1 & +24.3* & +0.4 & +18.0* & +12.6* & -168* & +8.5* & +11.1* & +8.1* & +22.1* & +8.7* & +11.1* & -0.05 & +0.20* & 36.0 & 4.2$\times$* \\
\textsc{MedGemma-27B} & Unwatermarked & 33.7 & 41.5 & 16.9 & 0.6 & 2.3 & 0 & 12.4 & 1.6 & 5.8 & 2.8 & 0.0 & 12.6 & 1.90 & 1.59 & -- & 1.0$\times$ \\
 & AAR & -0.9 & -3.0 & -0.8 & +1.5* & +1.9 & -43 & +2.6 & +2.9* & -0.7 & +2.6* & +0.1 & +0.1 & -0.08 & +0.06 & 19.5 & 1.6$\times$ \\
 & DipMark & +1.2 & -5.8 & -0.3 & +0.3 & -0.2 & -16 & +0.2 & +0.1 & -1.1 & +0.7 & +0.1 & -1.0 & -0.06 & +0.00 & 18.4 & 1.0$\times$ \\
 & KGW & -1.0 & +4.7 & +1.9 & +0.7 & +0.3 & -41 & +3.3 & +1.6 & +0.8 & +1.6 & +0.2 & +2.0 & -0.01 & +0.13 & 18.5 & 1.8$\times$* \\
 & PPL & -0.2 & +7.4 & +3.4 & +34.2* & +2.7* & -23 & +5.5* & +1.5 & +4.5* & +1.8 & +6.7* & 0.0 & -0.04 & +0.04 & 23.0 & 1.4$\times$ \\
 & SynthID & -0.3 & -1.9 & -0.8 & +1.5 & +1.3 & +3 & +2.7 & +0.9 & -0.3 & +0.3 & +0.2 & -1.0 & +0.01 & +0.00 & 22.8 & 0.9$\times$ \\
\textsc{Qwen-3-VL-8B} & Unwatermarked & 31.3 & 47.0 & 19.9 & 0.6 & 1.8 & 0 & 21.7 & 3.0 & 4.9 & 7.6 & 0.6 & 14.8 & 1.95 & 1.57 & -- & 1.0$\times$ \\
 & AAR & -4.3* & 0.0 & -5.2* & 0.0 & +2.5* & -3 & +1.3 & +0.6 & +0.7 & +7.3* & +0.6 & +4.3 & +0.06 & +0.07 & 22.2 & 1.8$\times$ \\
 & DipMark & -2.5 & +2.9 & -1.5 & -0.1 & +1.8 & +17 & +1.5 & +1.1 & +2.6 & +1.2 & -0.2 & -2.0 & +0.06 & -0.01 & 25.0 & 1.1$\times$ \\
 & KGW & -1.0 & +1.1 & +0.7 & +0.7 & +1.9 & +8 & +4.5 & +2.2 & +1.7 & +2.9 & +0.1 & +3.0 & +0.07 & +0.04 & 24.6 & 1.7$\times$ \\
 & PPL & -5.1* & +2.0 & -2.5 & +22.5* & +1.1 & -22 & -1.1 & +0.6 & +4.7* & +7.3* & +7.2* & -0.5 & -0.10 & -0.02 & 24.9 & 1.5$\times$ \\
 & SynthID & -4.5* & +3.1 & -2.1 & +0.1 & +1.4 & -9 & +2.0 & +1.9 & +0.6 & +6.2* & -0.4 & +3.9 & -0.04 & -0.00 & 24.5 & 1.0$\times$ \\
\textsc{Qwen-3-VL-32B} & Unwatermarked & 40.8 & 27.9 & 15.7 & 0.2 & 0.7 & 1 & 15.3 & 1.3 & 3.8 & 3.8 & 0.2 & 7.0 & 2.69 & 1.29 & -- & 1.0$\times$ \\
 & AAR & -3.0 & +3.1 & -0.7 & +1.5* & +1.9* & -2 & -1.1 & +0.3 & -0.1 & +0.5 & +3.0* & +0.6 & -0.01 & +0.02 & 15.4 & 0.6$\times$ \\
 & DipMark & -1.4 & +5.1 & +1.0 & +0.5 & +0.9 & -3 & -1.0 & +0.1 & 0.0 & +0.6 & +0.8 & +2.6 & -0.00 & +0.04 & 14.1 & 0.8$\times$ \\
 & KGW & -0.9 & +3.9 & -0.1 & +1.1 & +0.2 & +3 & +1.4 & +0.8 & -0.2 & +0.6 & +1.2* & +0.8 & +0.08 & +0.04 & 15.4 & 1.0$\times$ \\
 & PPL & -2.6 & +4.1 & -0.6 & +35.6* & +2.0* & -3 & +1.2 & -0.5 & +2.6* & +2.2 & +11.6* & +1.6 & +0.01 & +0.05 & 14.4 & 1.2$\times$ \\
 & SynthID & +1.1 & +3.9 & +2.5 & +1.2 & +2.3* & -9 & -0.4 & +0.9 & -0.4 & +0.7 & +3.5* & +0.7 & -0.04 & +0.08 & 15.3 & 1.6$\times$ \\
\bottomrule
\end{tabular}
\begin{tablenotes}
\footnotesize
\item Single-response axes (per $100$ questions where suffixed): ConfErr (confident error, on BOTH-CORRECT pairs), F\&C (faulty-but-correct: correct letter $+\geq 1$ defect), Spell/100, Fab/100 (fabricated entities), Contr (within-response contradiction), VigFab (vignette fabrication), Misread (clue misread), Fmt (format/termination failure), Ling (linguistic corruption), Misapp/100 (misapplied real terms). Image-grounding (multimodal): Sup, Con (per-question \textsc{supported}/\textsc{contradicted} visual claims), Net\% (relative change in $\textsc{supported}-\textsc{contradicted}$). Pairwise: Major\% (MAJOR divergence on BOTH-CORRECT pairs), FabRatio (WM/Base vignette-fabrication rate).
\end{tablenotes}
\end{threeparttable}
\end{sidewaystable}

==> data/main_combined.tex <==
\begin{table}[t]
\centering
\footnotesize
\setlength{\tabcolsep}{3pt}
\begin{threeparttable}
\caption{\textbf{Reasoning damage at $99\%$ TPR}, two most-affected models per benchmark (full grids in \cref{app:full_judge_tables}). Scheme rows are paired-bootstrap $\Delta$ vs.\ the unwatermarked baseline; VigFab is a WM/Base ratio and Major\% is absolute. $^{*}\,p<0.01$ (sign-flip permutation, $n{=}5000$); ``--'': base rate too low for a stable ratio.}\label{tab:main_combined}
\begin{tabular}{llrrrrrrr}
\toprule
Model & Scheme & $\Delta$Acc & Fab/100 & Misapp/100 & Spell/100 & VigFab & F\&C & Major\% \\
\midrule
\multicolumn{9}{l}{\textit{MedQA}} \\
\textsc{Phi-4-14B} & Unwatermarked & 81.4 & 0.3 & 9.8 & 0.1 & 1.0$\times$ & 11.4 & -- \\
 & AAR & -2.5 & +1.8* & +3.8* & +1.5* & 14.0$\times$* & +6.5* & 1.9 \\
 & DipMark & -0.9 & +0.1 & +2.0 & +0.3 & 0.8$\times$ & +3.6* & 2.8 \\
 & KGW & -0.7 & +1.5* & +3.2 & +2.2* & 3.0$\times$* & +9.5* & 3.6 \\
 & PPL & -8.6* & +3.8* & +3.8 & +69.6* & 18.0$\times$* & +9.6* & 2.3 \\
 & SynthID & -3.2* & +6.6* & +7.2* & +10.6* & 7.6$\times$* & +14.9* & 3.3 \\
\textsc{OpenBioLLM-70B} & Unwatermarked & 73.6 & 0.0 & 10.9 & 0.6 & 1.0$\times$ & 12.9 & -- \\
 & AAR & -0.2 & +0.9* & +0.5 & +0.9 & 0.9$\times$ & +4.4* & 4.4 \\
 & DipMark & -1.1 & +0.4 & -0.4 & +0.3 & 1.1$\times$ & +1.5 & 3.2 \\
 & KGW & -17.4* & +1.9* & +3.8 & +5.2* & 3.5$\times$* & +4.2* & 5.6 \\
 & PPL & -7.7* & +2.1* & -0.1 & +51.5* & 1.9$\times$ & +6.7* & 6.6 \\
 & SynthID & -11.4* & +13.6* & +5.3* & +25.9* & 6.6$\times$* & +14.6* & 8.7 \\
\multicolumn{9}{l}{\textit{MedXpertQA-MM}} \\
\textsc{MedGemma-4B} & Unwatermarked & 24.1 & 1.9 & 16.5 & 1.0 & 1.0$\times$ & 16.5 & -- \\
 & AAR & -1.0 & +6.5* & +8.7* & +3.4* & 3.1$\times$* & +1.2 & 38.3 \\
 & DipMark & +0.2 & +0.7 & +1.4 & +0.2 & 1.2$\times$ & +1.6 & 35.0 \\
 & KGW & -2.6 & +8.9* & +11.8* & +15.4* & 3.1$\times$* & +0.6 & 31.7 \\
 & PPL & -1.7 & +6.0* & +4.5 & +43.6* & 2.1$\times$* & 0.0 & 34.7 \\
 & SynthID & -3.1 & +12.6* & +11.1* & +18.0* & 4.2$\times$* & +0.4 & 36.0 \\
\textsc{Lingshu-7B} & Unwatermarked & 23.9 & 1.5 & 17.6 & 0.4 & 1.0$\times$ & 13.7 & -- \\
 & AAR & -0.5 & +12.9* & +3.5 & +5.4* & 2.8$\times$* & +3.7 & 33.0 \\
 & DipMark & +1.0 & +0.3 & +0.5 & +0.1 & 1.0$\times$ & +1.4 & 22.6 \\
 & KGW & -0.8 & +13.2* & +12.2* & +16.2* & 3.6$\times$* & +6.0 & 42.9 \\
 & PPL & -0.6 & +3.9* & -1.3 & +37.9* & 2.4$\times$* & +2.3 & 20.0 \\
 & SynthID & -2.1 & +39.2* & +12.0* & +18.9* & 7.0$\times$* & +5.5* & 30.5 \\
\bottomrule
\end{tabular}
\end{threeparttable}
\end{table}


==> data/ppl_tables_medqa.tex <==
% =============================================================
% MedQA watermark perplexity table -- merged across all 7 models.
% Manually compacted from the per-model auto-generated tables.
% Saturation rule applied per (model, scheme): keep configurations up
% to and including the first one with TPR >= 99%; subsequent stronger
% configurations are dropped (---). Schemes that never reach 99% TPR
% retain all evaluated configurations.
% Required packages: booktabs, makecell, rotating (sidewaystable), float.
% =============================================================

\begin{sidewaystable}[p]
\centering
\caption{MedQA: watermark detectability (TPR @ 1\%FPR, in \%) and generation perplexity shift ($\Delta$PPL\,$=$\,PPL$_{\mathrm{wm}}-$PPL$_{\mathrm{base}}$) for every (model, scheme, strength) configuration evaluated in \cref{sec:accuracy}, computed over $N=2000$ questions (full benchmark). Per-model unwatermarked baseline PPL is shown beneath each model header. For each (model, scheme) we report all configurations up to and including the first one with TPR\,$\geq$\,99\%; stronger configurations beyond that saturation point are omitted (---), as they yield no additional detectability.}
\label{tab:medqa_ppl_all}
\footnotesize
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.05}
\begin{tabular}{ll *{6}{rr}}
\toprule
 & & \multicolumn{2}{c}{\makecell{\textsc{Gemma-3-12B}\\(1.38)}}
   & \multicolumn{2}{c}{\makecell{\textsc{Llama-3.1-70B}\\(1.18)}}
   & \multicolumn{2}{c}{\makecell{\textsc{Llama-3.1-8B}\\(1.58)}}
   & \multicolumn{2}{c}{\makecell{\textsc{OpenBioLLM-70B}\\(1.30)}}
   & \multicolumn{2}{c}{\makecell{\textsc{Phi-4-14B}\\(1.30)}}
   & \multicolumn{2}{c}{\makecell{\textsc{UltraMedical-70B}\\(1.39)}} \\
\cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8} \cmidrule(lr){9-10} \cmidrule(lr){11-12} \cmidrule(lr){13-14}
Scheme & Strength
 & TPR & $\Delta$PPL & TPR & $\Delta$PPL & TPR & $\Delta$PPL & TPR & $\Delta$PPL
 & TPR & $\Delta$PPL & TPR & $\Delta$PPL \\
\midrule
AAR & $\delta=0$    & 96.3 & $+$0.00 & 37.3 & $-$0.00 & 91.4 & $-$0.01 & 36.6 & $-$0.02 & 70.0 & $+$0.00 & 67.8 & $-$0.03 \\
AAR & $\delta=0.1$  & 98.2 & $+$0.05 & 47.1 & $+$0.02 & 95.7 & $+$0.11 & 45.3 & $+$0.01 & ---  & ---     & 76.5 & $+$0.01 \\
AAR & $\delta=0.2$  & 99.3 & $+$0.10 & 55.6 & $+$0.04 & 98.1 & $+$0.32 & 51.7 & $+$0.05 & 86.0 & $+$0.10 & 84.4 & $+$0.05 \\
AAR & $\delta=0.3$  & ---  & ---     & 64.7 & $+$0.06 & 99.4 & $+$6.95 & 59.1 & $+$0.10 & 92.0 & $+$0.18 & 90.5 & $+$0.11 \\
AAR & $\delta=0.4$  & ---  & ---     & 73.1 & $+$0.09 & ---  & ---     & 66.7 & $+$0.16 & 96.2 & $+$0.30 & 93.5 & $+$0.17 \\
AAR & $\delta=0.5$  & ---  & ---     & 80.7 & $+$0.13 & ---  & ---     & 76.1 & $+$0.24 & 98.1 & $+$0.51 & 95.6 & $+$0.25 \\
\midrule
DipMark & $\alpha=0.5$ & 90.1 & $+$0.09 & 30.2 & $+$0.04 & 83.8 & $+$0.23 & 25.4 & $+$0.06 & 59.8 & $+$0.09 & 57.7 & $+$0.08 \\
\midrule
KGW & $\delta=0.5$ & 16.9 & $+$0.01 &  6.4 & $+$0.01 & 18.6 & $+$0.02 &  3.1 & $+$0.01 &  5.9 & $+$0.01 & 11.7 & $+$0.01 \\
KGW & $\delta=1$   & 65.1 & $+$0.04 & 22.2 & $+$0.02 & 63.0 & $+$0.09 & 11.4 & $+$0.03 & 27.5 & $+$0.04 & 41.2 & $+$0.04 \\
KGW & $\delta=2$   & 99.4 & $+$0.17 & 70.7 & $+$0.09 & 99.2 & $+$0.43 & 51.4 & $+$0.14 & 87.3 & $+$0.19 & 91.4 & $+$0.18 \\
KGW & $\delta=3$   & ---  & ---     & 95.2 & $+$0.23 & ---  & ---     & 85.5 & $+$0.35 & 99.2 & $+$0.56 & 99.1 & $+$0.43 \\
KGW & $\delta=4$   & ---  & ---     & 99.1 & $+$0.44 & ---  & ---     & 95.9 & $+$0.71 & ---  & ---     & ---  & ---     \\
KGW & $\delta=5$   & ---  & ---     & ---  & ---     & ---  & ---     & 98.8 & $+$1.26 & ---  & ---     & ---  & ---     \\
\midrule
PPL & $\varepsilon=0$   & 99.5 & $+$0.07 & 81.7 & $+$0.12 & 99.1 & $+$0.07 & 57.2 & $+$0.07 & 90.8 & $+$0.11 & 94.4 & $+$0.14 \\
PPL & $\varepsilon=0.1$ & ---  & ---     & 92.8 & $+$0.17 & ---  & ---     & 73.9 & $+$0.15 & 96.7 & $+$0.19 & 97.7 & $+$0.22 \\
PPL & $\varepsilon=0.2$ & ---  & ---     & 97.8 & $+$0.26 & ---  & ---     & 86.6 & $+$0.28 & ---  & ---     & 99.3 & $+$0.36 \\
PPL & $\varepsilon=0.3$ & ---  & ---     & 99.3 & $+$0.45 & ---  & ---     & 92.7 & $+$0.42 & 99.8 & $+$0.57 & ---  & ---     \\
PPL & $\varepsilon=0.4$ & ---  & ---     & ---  & ---     & ---  & ---     & 95.4 & $+$0.55 & ---  & ---     & ---  & ---     \\
PPL & $\varepsilon=0.5$ & ---  & ---     & ---  & ---     & ---  & ---     & 97.5 & $+$0.72 & ---  & ---     & ---  & ---     \\
\midrule
SynthID & $\ell=2$ & 91.1 & $-$0.04 & 38.3 & $-$0.02 & 85.9 & $-$0.11 & 22.9 & $-$0.03 & 48.4 & $-$0.04 & 67.4 & $-$0.03 \\
SynthID & $\ell=3$ & 98.9 & $+$0.16 & 63.9 & $+$0.07 & 98.3 & $+$0.42 & 48.1 & $+$0.13 & 84.5 & $+$0.17 & 89.2 & $+$0.15 \\
SynthID & $\ell=4$ &100.0 & $+$0.47 & 79.4 & $+$0.18 &100.0 & $+$4.14 & 70.5 & $+$0.35 & 97.2 & $+$0.64 & 96.3 & $+$0.41 \\
SynthID & $\ell=5$ & ---  & ---     & 87.9 & $+$0.31 & ---  & ---     & 83.5 & $+$0.74 & 99.1 & $+$1.62 & 98.8 & $+$0.88 \\
SynthID & $\ell=6$ & ---  & ---     & 93.4 & $+$0.49 & ---  & ---     & 93.3 & $+$1.79 & ---  & ---     & 99.2 & $+$4.41 \\
\bottomrule
\end{tabular}
\end{sidewaystable}


==> data/ppl_tables_medxpertqa_mm.tex <==
% =============================================================
% MedXpertQA-MM watermark perplexity table -- merged across all 7 models.
% Manually compacted from the per-model auto-generated tables.
% Saturation rule applied per (model, scheme): keep configurations up
% to and including the first one with TPR >= 99%; subsequent stronger
% configurations are dropped (---). Schemes that never reach 99% TPR
% retain all evaluated configurations.
% Required packages: booktabs, makecell, rotating (sidewaystable), float.
% =============================================================

\begin{sidewaystable}[p]
\centering
\caption{MedXpertQA-MM: watermark detectability (TPR @ 1\%FPR, in \%) and generation perplexity shift ($\Delta$PPL\,$=$\,PPL$_{\mathrm{wm}}-$PPL$_{\mathrm{base}}$) for every (model, scheme, strength) configuration evaluated in \cref{sec:accuracy}, computed over $N=2000$ questions (full benchmark). Per-model unwatermarked baseline PPL is shown beneath each model header. For each (model, scheme) we report all configurations up to and including the first one with TPR\,$\geq$\,99\%; stronger configurations beyond that saturation point are omitted (---), as they yield no additional detectability.}
\label{tab:medxpertqa_mm_ppl_all}
\footnotesize
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.05}
\begin{tabular}{ll *{7}{rr}}
\toprule
 & & \multicolumn{2}{c}{\makecell{\textsc{Gemma-4-31B}\\(3.25)}}
   & \multicolumn{2}{c}{\makecell{\textsc{Lingshu-32B}\\(1.46)}}
   & \multicolumn{2}{c}{\makecell{\textsc{Lingshu-7B}\\(1.51)}}
   & \multicolumn{2}{c}{\makecell{\textsc{MedGemma-27B}\\(1.33)}}
   & \multicolumn{2}{c}{\makecell{\textsc{MedGemma-4B}\\(1.50)}}
   & \multicolumn{2}{c}{\makecell{\textsc{Qwen-3-VL-32B}\\(1.43)}}
   & \multicolumn{2}{c}{\makecell{\textsc{Qwen-3-VL-8B}\\(1.48)}} \\
\cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8} \cmidrule(lr){9-10} \cmidrule(lr){11-12} \cmidrule(lr){13-14} \cmidrule(lr){15-16}
Scheme & Strength
 & TPR & $\Delta$PPL & TPR & $\Delta$PPL & TPR & $\Delta$PPL & TPR & $\Delta$PPL
 & TPR & $\Delta$PPL & TPR & $\Delta$PPL & TPR & $\Delta$PPL \\
\midrule
AAR & $\delta=0$    & 65.2 & $+$0.02 & 72.6 & $+$0.02 & 73.7 & $+$0.02 & 90.0 & $+$0.00 & 84.2 & $-$0.07 & 93.5 & $-$0.01 & 97.9 & $-$0.04 \\
AAR & $\delta=0.1$  & 71.2 & $+$0.08 & 82.5 & $+$0.08 & 82.9 & $+$0.09 & 94.2 & $+$0.04 & 91.2 & $-$0.01 & 95.5 & $+$0.03 & 98.6 & $+$0.03 \\
AAR & $\delta=0.2$  & 79.5 & $+$0.12 & 89.5 & $+$0.19 & 91.4 & $+$0.19 & 96.6 & $+$0.09 & 94.0 & $+$0.10 & 97.9 & $+$0.09 & 99.1 & $+$0.11 \\
AAR & $\delta=0.3$  & 84.8 & $+$0.17 & 93.8 & $+$0.33 & 94.5 & $+$0.33 & 98.0 & $+$0.15 & 96.8 & $+$0.23 & 98.9 & $+$0.15 & ---  & ---     \\
AAR & $\delta=0.4$  & 90.5 & $+$0.29 & 96.2 & $+$0.56 & 97.5 & $+$0.55 & 98.9 & $+$0.22 & 98.2 & $+$0.43 & 99.5 & $+$0.23 & ---  & ---     \\
AAR & $\delta=0.5$  & 92.8 & $+$0.41 & 98.3 & $+$1.40 & 98.5 & $+$3.22 & 99.6 & $+$0.34 & 99.0 & $+$0.77 & ---  & ---     & ---  & ---     \\
\midrule
DipMark & $\alpha=0.5$ & 45.6 & $+$0.14 & 57.0 & $+$0.13 & 57.5 & $+$0.13 & 82.0 & $+$0.07 & 72.5 & $+$0.16 & 87.1 & $+$0.09 & 94.5 & $+$0.12 \\
\midrule
KGW & $\delta=0.5$ &  7.1 & $+$0.00 &  9.2 & $+$0.01 & 10.1 & $+$0.02 & 14.8 & $+$0.01 & 14.1 & $+$0.01 & 17.1 & $+$0.01 & 30.3 & $+$0.02 \\
KGW & $\delta=1$   & 26.9 & $+$0.09 & 34.1 & $+$0.06 & 38.9 & $+$0.06 & 59.2 & $+$0.04 & 54.0 & $+$0.06 & 62.3 & $+$0.04 & 81.2 & $+$0.07 \\
KGW & $\delta=2$   & 81.0 & $+$0.29 & 91.0 & $+$0.25 & 91.0 & $+$0.24 & 97.0 & $+$0.16 & 91.8 & $+$0.26 & 98.0 & $+$0.17 & 99.2 & $+$0.26 \\
KGW & $\delta=3$   & 96.9 & $+$0.58 & 99.2 & $+$0.66 & 99.0 & $+$0.57 &100.0 & $+$0.39 & 96.5 & $+$0.66 & 99.9 & $+$0.40 & ---  & ---     \\
KGW & $\delta=4$   & 99.9 & $+$1.05 & ---  & ---     & ---  & ---     & ---  & ---     & ---  & ---     & ---  & ---     & ---  & ---     \\
KGW & $\delta=5$   & ---  & ---     & ---  & ---     & ---  & ---     & ---  & ---     & 97.2 & $+$2.26 & ---  & ---     & ---  & ---     \\
\midrule
PPL & $\varepsilon=0$   & 88.9 & $+$0.19 & 92.8 & $+$0.07 & 94.7 & $+$0.06 & 98.6 & $+$0.07 & 91.1 & $+$0.03 & 99.1 & $+$0.06 & 99.6 & $+$0.04 \\
PPL & $\varepsilon=0.1$ & 96.1 & $+$0.32 & 97.8 & $+$0.17 & 97.4 & $+$0.15 & 99.7 & $+$0.15 & ---  & ---     & ---  & ---     & ---  & ---     \\
PPL & $\varepsilon=0.2$ & 98.8 & $+$0.59 & 99.4 & $+$0.34 & 99.2 & $+$0.30 & ---  & ---     & 94.0 & $+$0.25 & ---  & ---     & ---  & ---     \\
PPL & $\varepsilon=0.3$ & 99.6 & $+$0.89 & ---  & ---     & ---  & ---     & ---  & ---     & ---  & ---     & ---  & ---     & ---  & ---     \\
PPL & $\varepsilon=0.4$ & ---  & ---     & ---  & ---     & ---  & ---     & ---  & ---     & 96.4 & $+$0.54 & ---  & ---     & ---  & ---     \\
PPL & $\varepsilon=0.5$ & ---  & ---     & ---  & ---     & ---  & ---     & ---  & ---     & 96.7 & $+$0.73 & ---  & ---     & ---  & ---     \\
\midrule
SynthID & $\ell=2$ & 61.2 & $-$0.01 & 63.3 & $-$0.07 & 69.0 & $-$0.07 & 92.9 & $+$0.02 & 88.6 & $-$0.04 & 89.0 & $-$0.05 & 94.8 & $-$0.09 \\
SynthID & $\ell=3$ & 81.2 & $+$0.28 & 89.6 & $+$0.22 & 92.5 & $+$0.21 & 98.7 & $+$0.23 & 95.0 & $+$0.34 & 98.1 & $+$0.15 & 99.4 & $+$0.18 \\
SynthID & $\ell=4$ & 90.7 & $+$0.67 & 98.0 & $+$0.96 & 98.0 & $+$0.79 & 99.9 & $+$0.59 & 96.5 & $+$1.06 & 99.5 & $+$0.40 & ---  & ---     \\
SynthID & $\ell=5$ & 95.4 & $+$1.08 & 99.4 & $+$3.89 & 99.8 & $+$3.00 & ---  & ---     & 96.6 & $+$2.07 & ---  & ---     & ---  & ---     \\
\bottomrule
\end{tabular}
\end{sidewaystable}


==> headers/lqa/colors.tex <==
% Description: This file contains a few useful colors.
%
% Usage: You may need to comment out the usepackage command below, if they
% conflict with your conference template


%%%%%%%%%
% SETUP %
%%%%%%%%%
% import relevant packages

% Comment out the following line in case of error "Option clash for package color"
\usepackage[usenames, dvipsnames]{color} % for textcolor
\usepackage{xcolor} % for definecolor


%%%%%%%%%%%%%%%%%%%%%%
%  MATPLOTLIB COLORS %
%%%%%%%%%%%%%%%%%%%%%%


% blue
\definecolor{my-full-blue}{HTML}{1F77B4}
%\definecolor{blue}{RGB}{31,119,180} 

% orange
\definecolor{my-full-orange}{HTML}{FF7F0E}
%\definecolor{orange}{RGB}{255,127,14}

% green
\definecolor{my-full-green}{HTML}{2CA02C}
%\definecolor{green}{RGB}{44,160,44}

% red
\definecolor{my-full-red}{HTML}{d62728}
%\definecolor{red}{RGB}{214,39,40}

% purple
\definecolor{my-full-purple}{HTML}{9467bd}
%\definecolor{purple}{RGB}{148,103,189}

% brown
\definecolor{my-full-brown}{HTML}{8c564b}
%\definecolor{brown}{RGB}{140,86,75}

% pink
\definecolor{my-full-pink}{HTML}{e377c2}
%\definecolor{pink}{RGB}{227,119,194}

% gray
\definecolor{my-full-gray}{HTML}{7f7f7f}
%\definecolor{gray}{RGB}{127,127,127}

% olive
\definecolor{my-full-olive}{HTML}{bcbd22}
%\definecolor{olive}{RGB}{188,189,34}

% cyan
\definecolor{my-full-cyan}{HTML}{17becf}
%\definecolor{cyan}{RGB}{23,190,207}

% lighter shades
\colorlet{my-blue}{my-full-blue!30}
\colorlet{my-orange}{my-full-orange!30}
\colorlet{my-green}{my-full-green!30}
\colorlet{my-red}{my-full-red!30}
\colorlet{my-purple}{my-full-purple!30}
\colorlet{my-brown}{my-full-brown!30}
\colorlet{my-pink}{my-full-pink!30}
\colorlet{my-gray}{my-full-gray!30}
\colorlet{my-olive}{my-full-olive!30}
\colorlet{my-cyan}{my-full-cyan!30}

%%%%%%%%%%%%%%%%%%%%%%
%  PROJECT-SPECIFIC  %
%%%%%%%%%%%%%%%%%%%%%%


==> headers/lqa/csvsimple.tex <==
% Description: This file enables displaying csv tables
%
% Usage: \input{headers/lqa/csvsimple}

\usepackage{csvsimple}

% EXAMPLE USAGE

% \begin{table}
% 	\begin{tabular}{ll}
% 		A & B \\
% 		\hline
% 		\csvreader[%
% 			head to column names,
% 			late after line=\\,
% 			separator=semicolon
% 		]{algorithms.csv}{}{%
% 			\a & \b
% 		}
% 	\end{tabular}
% 	\caption{Caption.}
% 	\label{tab:label}
% \end{table}

==> headers/lqa/headings.tex <==
% Description: This file defines headings
%
% Usage: \input{headers/lqa/headings}

\makeatletter

% for IEEE:
% replace trailing : by trailing .
\def\@IEEEsectpunct{.\ }

% Definition for paragraphs, handling spacing correctly
% https://tex.stackexchange.com/questions/31780/where-can-i-find-help-files-or-documentation-for-commands-like-startsection-fo
% http://joshua.smcvt.edu/latex2e/bs-at-startsection.html
\def\para{\@startsection%
	{paragraph}% 
	{4}% level
	{0\parindent}% indent
	{0.6ex plus 0.1ex minus 0.1ex}% beforeskip
	{0ex}% afterskip
	{\normalfont\normalsize\itshape\bfseries}% style
	*% do not number
}%

\makeatother


% Alternatively: Define \para in terms of \paragraph
% \newcommand{\para}[1]{\paragraph{#1.}}

==> headers/lqa/subfigures.tex <==
% Description: This file introduces a subfigure which correctly aligns
% captions
%
% Usage:
% - \input{headers/lqa/subfigures}
% - You may need to comment out the usepackage command below in case of
%   conflicts

% EXAMPLE USAGE:
%
% \begin{figure}
% 	\centering
% 	\mysubfigure[0.49\linewidth]{
% 		\centering
% 		Content of subfigure 1
% 	}{Caption of subfigure\label{fig:subfig1}}
% 	\mysubfigure[0.49\linewidth]{
% 		\centering
% 		Content of subfigure 2
% 	}{Caption of subfigure\label{fig:subfig2}}
% 	\caption{An example of subfigures.}
% 	\label{fig:subfigures}
% \end{figure}

%%%%%%%%%%%%%%
% USEPACKAGE %
%%%%%%%%%%%%%%
\usepackage{subcaption}

%%%%%%%%%%%
% COMMAND %
%%%%%%%%%%%

\newcommand{\mysubfigure}[3][\linewidth]{\subcaptionbox{#3}[#1]{
	\begin{minipage}{#1}
		% uses minipage to prevent unexpected interactions,
		% e.g., for align
		#2
	\end{minipage}
}}


==> headers/lqa/tikz.tex <==
% Description: This file contains a few useful tikz libraries.
%
% Usage: \input{headers/lqa/tikz}

%%%%%%%%%
% SETUP %
%%%%%%%%%
% import relevant package
\usepackage{tikz}

%%%%%%%%%%%%%%%%%%%%%%
%  PROJECT-SPECIFIC  %
%%%%%%%%%%%%%%%%%%%%%%
% adapt the following list of libraries as required

\usetikzlibrary{arrows}
\usetikzlibrary{automata}
\usetikzlibrary{calc}
\usetikzlibrary{backgrounds}
\usetikzlibrary{decorations.markings}
\usetikzlibrary{decorations.pathmorphing}
\usetikzlibrary{decorations.pathreplacing}
\usetikzlibrary{fit}
\usetikzlibrary{patterns}
\usetikzlibrary{positioning}
\usetikzlibrary{shadows}
\usetikzlibrary{shapes}
\usetikzlibrary{shapes.geometric}








==> tables/judge_table.tex <==

\begin{table}[t]
    \centering
    \caption{Overview of reasoning-quality audits. Each audit targets a distinct facet of reasoning integrity; together they cover per-response error detection, paired divergence, and reasoning-trace analysis.}
    \label{tab:audit_overview}
    \small
    \begin{tabular}{@{}p{1.9cm}p{2.0cm}p{2.0cm}p{5.7cm}@{}}
        \toprule
        \textbf{Audit}          & \textbf{Models} & \textbf{Benchmark}   & \textbf{What it measures}                                                                                                                                                                            \\
        \midrule
        Single-response (blind) & Non-thinking    & MedQA, MedXpertQA-MM & Per-response error flags: terminology corruption, vignette fabrication, self-contradiction, confident errors, clue misreads, format failures; plus image-grounding claims for the multimodal variant \\[4pt]
        Pairwise divergence     & Non-thinking    & MedQA, MedXpertQA-MM & Correctness configuration, diagnostic interpretation divergence (None/Minor/Major)                                                                                                                   \\[4pt]
        Reasoning-trace         & Thinking        & MedQA                & Six relative-change dimensions (e.g.\ reasoning coherence, terminological precision) each scored from $-2$ (test response substantially worse than reference) through $0$ (comparable) to $+2$ (substantially better); absolute clinical-deployment ratings (safety, supervisory burden); primary degradation pattern \\
        \bottomrule
    \end{tabular}
\end{table}
